Visual Attention Emerges from Recurrent Sparse Reconstruction

Visual attention helps achieve robust perception under noise, corruption, and distribution shifts in human vision, which are areas where modern neural networks still fall short. We present VARS, Visual Attention from Recurrent Sparse reconstruction, a new attention formulation built on two prominent features of the human visual attention mechanism: recurrency and sparsity. Related features are grouped together via recurrent connections between neurons, with salient objects emerging via sparse regularization. VARS adopts an attractor network with recurrent connections that converges toward a stable pattern over time. Network layers are represented as ordinary differential equations (ODEs), formulating attention as a recurrent attractor network that equivalently optimizes the sparse reconstruction of input using a dictionary of "templates" encoding underlying patterns of data. We show that self-attention is a special case of VARS with a single-step optimization and no sparsity constraint. VARS can be readily used as a replacement for self-attention in popular vision transformers, consistently improving their robustness across various benchmarks. Code is released on GitHub (https://github.com/bfshi/VARS).

==> 2.5_toy_example.tex <==
\section{Neurons with Orientation Tuning: A Toy Example}
\label{sec:toy_example}

\baifeng{Xin suggested this section may be confusing with all the terminology from neuroscience community, so maybe we should delete this part or put it elsewhere. The Method Section should be self-contained and this part could be \textbf{skipped}.}


\begin{figure*}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=1.4\columnwidth]{figs/bars.png}}
\caption{\textit{(a)} An image of bars distributed on a regular spatial grid, with different orientation $\theta$. \textit{(b)} The bars in the middle are more salient because they constitute a contour (darker means giving higher output). \textit{(c, d)} The same contour will no longer be salient if it is just a part of the uniform texture. Lighter color means the output is suppressed.}
\label{fig:bars}
\end{center}
\vskip -0.2in
\end{figure*}

To first intuitively explain the relationship between neuronal recurrency and visual attention, we borrow the example of orientation-tuned neurons from ~\citet{zhaoping2014understanding}.
Assume we have an input image consist of bars with the same contrast but different orientations, each centered on a regular spatial grid (Fig.~\ref{fig:bars}(a)). Despite the equal contrast, the bars in the middle appear more salient to human eyes and automatically gain more attention than other bars because they constitute a contour (Fig.~\ref{fig:bars}(b)). In the mean time, such saliency will disappear if the contour is just a part of some uniform texture (Fig~\ref{fig:bars}(c)). Such behavior of feature selectivity is believed to be based on long-range recurrent connection~\cite{stettler2002lateral,gilbert1989columnar,bosking1997orientation,li1998neural,lamme2000distinct}, which we will briefly introduce in the following.

Consider a set of neurons distributed at each position in the grid and tuned to different orientations of the input bar in the same position. \xin{A set of neurons is defined as $\mathcal{N} = {n_{i,j}^c, c= 1, \dots C}\in\mathbb{R}^C$, where $C$ is the number of channels? What about a FC layer then?}

Each neuron maintains an internal state (membrane potential) which evolves by certain dynamics depending on the input. Then the output is a function of the internal state when it comes to an equilibrium. For simplicity, we assume the function is identity, \ie, the output equals the equilibrium state. We denote by $\mathbf{z}_{i\theta}$ the internal state of the neuron at position $i = (m, n)$ and tuned to orientation $\theta$. Then the dynamics of $\mathbf{z}$ is described by the following (simplified) differential equation:
\begin{equation}\small
\label{eq:toy_ode_wo_rec}
    \dv{\mathbf{z}_{i\theta}}{t} = -\mathbf{z}_{i\theta} + \mathbf{b}_{i\theta},
\end{equation}
where the two terms on RHS model the leakage current and the input, respectively. The input $\mathbf{b}_{i\theta}$ equals a positive constant $b$ if there exists a bar with orientation $\theta$ positioned at $i$, and zero otherwise. The final output of the neuron is the equilibrium state of Eq.~\ref{eq:toy_ode_wo_rec}.

We can see that the equilibirum state $\mathbf{z}^\ast_{i\theta}$ is identical to the input, \ie, $\mathbf{z}^\ast_{i\theta} = \mathbf{b}_{i\theta}$, which means each bar in the image will activate the corresponding neuron equally and give the same output value. However, the selective attention is missing, where the bars in the middle should be more salient (giving higher output value) since they form a complete contour (Fig.~\ref{fig:bars}(b)). In fact, this can be achieved by adding recurrent connections into Eq.~\ref{eq:toy_ode_wo_rec}:
\begin{equation}\small
    \dv{\mathbf{z}_{i\theta}}{t} = -\mathbf{z}_{i\theta} + \sum_{j \theta^\prime} \mathbf{A}_{i\theta, j\theta^\prime} \mathbf{z}_{j\theta^\prime} +  \mathbf{z}_{i\theta},
\end{equation}
where $\mathbf{A}$ is the weight of recurrent connection, and $\mathbf{A}_{i\theta, j\theta^\prime} \mathbf{z}_{j\theta^\prime}$ models the recurrent input from $\mathbf{z}_{j\theta^\prime}$ to $\mathbf{z}_{i\theta}$. To amplify the output from the middle contour, we can design the recurrent connection $\mathbf{A}$ so that there is mutual excitement between vertical bars aligned with each other:
\begin{equation}\small
    \mathbf{A}_{i\theta, j\theta^\prime} = 
    \begin{cases*}
        \alpha / 2, & if  $\theta = \theta^\prime = 0$, \ $j = i \pm (1, 0)$,  \\
        0, & otherwise.
    \end{cases*} 
\end{equation}


Now the neurons in the middle will receive an additional input from the output of its neighbors top and down. By symmetry, all the neurons in the middle line should have the same output $z$ (assuming the image is boundless). Then the output $z$ evolves by
\begin{equation}\small
    \dv{z}{t} = -z + \alpha z + b,
\end{equation}
and converges to $z^\ast = \frac{b}{1 - \alpha}$. In this way, the output from the middle contour is amplified by the factor $\frac{1}{1 - \alpha}$ (assuming $\alpha < 1$). Meanwhile, other random bars do not receive the recurrent input and thus keeps the output identical to the input value $b$. In this way, the contour becomes relatively more salient than other meaningless random patterns.

On the other hand, the saliency will disappear if the contour is just part of the uniform texture (Fig.~\ref{fig:bars}(c)). This is achieved by adding mutual inhibition between vertical bars that are not aligned with, but parallel to each other:
\begin{equation}\small
    \mathbf{A}_{i\theta, j\theta^\prime} = 
    \begin{cases*}
        \alpha / 2, & if  $\theta = \theta^\prime = 0$, \ $j = i \pm (1, 0)$,  \\
        -\beta / 2, & if  $\theta = \theta^\prime = 0$, \ $j = i \pm (0, 1)$,  \\
        0, & otherwise.
    \end{cases*} 
\end{equation}
Now if we further assume by symmetry that each bar in the image gives the same output $z$ , then $z$ evolves by
\begin{equation}\small
    \dv{z}{t} = -z + (\alpha - \beta) z + b,
\end{equation}
which gives the final output $z^\ast = \frac{b}{1 - \alpha + \beta}$. When $\beta > \alpha$, there is no saliency and the whole texture is suppressed (Fig.~\ref{fig:bars}(d)).

Apparently, what patterns are amplified or suppressed in the network is totally decided by the design of recurrent connection $\mathbf{A}$. Unfortunately, manually designing it as in the previous example seems unrealistic for general visual system like DNNs. So can we learn the recurrent connection from natural images? We will first generalize the human-like attention into deep neural networks in the next section, and then go back to this question in Sec.~\ref{sec:sparse_recon}.



